Identification and Verification of Attack-Tree Threat Models in Connected Vehicles

As a result of the ever-increasing application of cyber-physical components in the automotive industry, cybersecurity has become an urgent topic. Adapting technologies and communication protocols like Ethernet and WiFi in connected vehicles yields many attack scenarios. Consequently, ISO/SAE 21434 and UN R155 (2021) define a standard and regulatory framework for automotive cybersecurity. Both documents follow a risk management-based approach and require a threat modeling methodology for risk analysis and identification. Such a threat modeling methodology must conform to the Threat Analysis and Risk Assessment (TARA) framework of ISO/SAE 21434. Conversely, existing threat modeling methods enumerate isolated threats disregarding the vehicle's design and connections. Consequently, they neglect the role of attack paths from a vehicle's interfaces to its assets. In other words, they are missing the TARA work products, e.g., attack paths compromising assets or feasibility and impact ratings. We propose a threat modeling methodology to construct attack paths by identifying, sequencing, and connecting vulnerabilities from a valid attack surface to an asset. Initially, we transform cybersecurity guidelines to attack trees, and then we use their formal interpretations to assess the vehicle's design. This workflow yields compositional construction of attack paths along with the required TARA work products (e.g., attack paths, feasibility, and impact). More importantly, we can apply the workflow iteratively in the context of connected vehicles to ensure design conformity, privacy, and cybersecurity. Finally, to show the complexity and the importance of preemptive threat identification and risk analysis in the automotive industry, we evaluate the presented model-based approach in a connected vehicle testing platform, SPIDER.

==> 00-preambles.tex <==
%%%%%%%%%%%%%%%%%
%%    MACROS.  %%
%%%%%%%%%%%%%%%%%
\makeatletter
\renewcommand\@biblabel[1]{#1. }
\makeatother

% Define "struts" as suggested by Claudio Beccari in
% a piece in TeX and TUG News, Vol. 2, 1993.
\newcommand\Tstrut{\rule{0pt}{4.6ex}}       % "top" strut
\newcommand\Bstrut{\rule[-0.9ex]{0pt}{0pt}} % "bottom" strut
\newcommand{\TBstrut}{\Tstrut\Bstrut} % top&bottom struts

%%% the following hides the section number while keeping their numbering for proper referencing in toc and \ref
\makeatletter
\def\@seccntformat#1{%
  \expandafter\csname c@#1\endcsname\c@section
  }
\makeatother

\def \wwgrant {This work was supported by the Austrian Research Promotion Agency (FFG) through project WhichWay (893075).}

%%%%%%%%%%%%%%%%%
%%  PACKAGES   %%
%%%%%%%%%%%%%%%%%
\usepackage{xcolor}
\colorlet{actcolor}{black}
\colorlet{comcolor}{orange}
\colorlet{envcolor}{cyan!50!blue!80!white}
\colorlet{infcolor}{green!50!black}
\colorlet{ecucolor}{red}
\colorlet{sencolor}{magenta}

\usepackage{balance}
\usepackage[english]{babel}

\usepackage{nameref}
\usepackage[square,sort,comma,numbers]{natbib}
% \setlength{\bibsep}{0pt plus 1pt minus 1pt}

\usepackage{amsmath,amssymb,amsfonts,amsthm}
\usepackage{stmaryrd}
\usepackage{graphicx}
\usepackage{array}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage[nice]{nicefrac}
\usepackage{siunitx}
\usepackage{eqnarray}
\usepackage{rotating}

\usepackage{float}
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{2}
\setcounter{totalnumber}{4}
\renewcommand{\topfraction}{0.85}
\renewcommand{\bottomfraction}{0.85}
\renewcommand{\textfraction}{0.15}
\renewcommand{\floatpagefraction}{0.8}
\renewcommand{\textfraction}{0.1}
\setlength{\floatsep}{10pt plus 5pt minus 10pt}
\setlength{\textfloatsep}{5pt plus 2pt minus 5pt}
% \setlength{\intextsep}{5pt plus 2pt minus 5pt}
\setlength{\intextsep}{5pt plus 2pt minus 5pt}

\usepackage{caption}
\usepackage{subcaption}
\captionsetup{font=footnotesize}
\captionsetup[table]{skip=0pt,aboveskip=0pt,belowskip=0pt}
\captionsetup[figure]{skip=0pt,aboveskip={3pt plus 5pt minus 5pt},belowskip={0pt plus 5pt minus 5pt}}
% \captionsetup[subfigure]{aboveskip=5pt,belowskip={2pt plus 0pt minus 5pt}}

\usepackage[usestackEOL]{stackengine}
\setstackgap{S}{0pt}

\usepackage[scaled=0.75]{beramono}
\usepackage[T1]{fontenc}

\pdfinclusionerrorlevel=1
\pdfminorversion=7

% enables the hyperref without colors and with bookmarks
\usepackage{hyperref}
\hypersetup{pdfauthor={Masoud Ebrahimi et al.},%
pdftitle={Identification and Verification of Attack-Tree Threat Models in Connected Vehicles},
pdfkeywords={Attack Paths, Smart Vehicles, Design Verification Expansion, Threat Identification},
breaklinks=true,
colorlinks=true,
linkcolor=black,
citecolor=black,
urlcolor=black,
pdfpagelayout=SinglePage,
pdfstartview=Fit}

\usepackage[capitalise]{cleveref}
\usepackage{xspace}
\xspaceaddexceptions{]\}}

\usepackage{enumitem}
\setlist[enumerate]{topsep=-2pt plus 2pt minus 2pt,itemsep=-1ex,partopsep=1ex,parsep=1ex}
\setlist[itemize]{topsep=-2pt plus 2pt minus 2pt,itemsep=-1ex,partopsep=1ex,parsep=1ex}

\setlength{\abovedisplayskip}{0.75\parskip}
\setlength{\belowdisplayskip}{0.75\parskip}
\setlength{\textfloatsep}{10pt plus 2.0pt minus 2.0pt}

%%%%%%%%%%%%%%%%%
%% Definitions %%
%%%%%%%%%%%%%%%%%
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
    T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

% Add a period to the end of an abbreviation unless there's one
% already, then \xspace.
\makeatletter
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\def\st{s.t\onedot}
\def\eg{e.g\onedot}
\def\ie{i.e\onedot}
\def\cf{c.f\onedot}
\def\etc{etc\onedot}
\def\vs{vs\onedot}
\def\wrt{w.r.t\onedot}
\def\dof{d.o.f\onedot}
\def\etal{et al\onedot}
\def\iso{ISO/SAE~21434\xspace}
\def\un{UN~R155\xspace}
\makeatother


%%%%%%%%%%%%%%%%%
%% Environments %%
%%%%%%%%%%%%%%%%%
\newtheoremstyle{theoremexample}% <name>
{\parskip}% <Space above>
{\parskip}% <Space below>
% {\upshape}% <Body font>
{\slshape}% <Body font>
{}% <Indent amount>
{\bfseries}% <Theorem head font>
{.}% <Punctuation after theorem head>
{.5em}% <Space after theorem headi>
{\thmname{#1}\thmnumber{ #2}\thmnote{\textnormal{ (#3)}}}
\theoremstyle{theoremexample}
\newtheorem{example}{Example}

\newtheoremstyle{theoremrunexample}% <name>
{\parskip}% <Space above>
{\parskip}% <Space below>
% {\upshape}% <Body font>
{\slshape}% <Body font>
{}% <Indent amount>
{\bfseries}% <Theorem head font>
{.}% <Punctuation after theorem head>
{.5em}% <Space after theorem headi>
{\thmname{#1}\thmnumber{ #2}\thmnote{\textnormal{ (#3)}}}
\theoremstyle{theoremrunexample}
\newtheorem{runexample}{Running Example}

%%%%%%%%%%%%%%%%%
%%   Commands  %%
%%%%%%%%%%%%%%%%%
% CUSTOM MACROS
\usepackage{alltt}
\let\oldalltt\alltt
\renewenvironment{alltt}{\vspace{-0.55\baselineskip}\begin{oldalltt}}{\end{oldalltt}\vspace{-0.1\baselineskip}}

\newcommand{\me}[1]{\textcolor{blue!50!red}{[\textbf{ME:}\xspace#1]}}
\newcommand{\quim}[1]{\textcolor{orange}{[\textbf{Quim:}\xspace#1]}}
\newcommand{\rb}[1]{\textcolor{green!50!black}{[\textbf{RB:}\xspace#1]}}
\newcommand{\cs}[1]{\textcolor{yellow!50!black}{[\textbf{CS:}\xspace#1]}}
\newcommand{\comment}[1]{}

% Colors
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\cyan}[1]{\textcolor{cyan!40!blue}{#1}}
\newcommand{\red}[1]{\textcolor{red!70!black}{#1}}
\newcommand{\purple}[1]{\textcolor{red!30!blue}{#1}}
\newcommand{\green}[1]{\textcolor{green!35!black}{#1}}
\newcommand{\type}[1]{\green{\texttt{#1}}\xspace}
\newcommand{\kw}[1]{\blue{\texttt{#1}}\xspace}
\newcommand{\field}[1]{\purple{\texttt{#1}}\xspace}
\newcommand{\val}[1]{\red{\texttt{#1}}\xspace}
\newcommand{\flow}{\kw{FLOW}}
\newcommand{\element}{\kw{ELEMENT}}
\newcommand{\boundary}{\kw{BOUNDARY}}
\newcommand{\connector}{\kw{CONNECTOR}}

% Boolean Connectives
\newcommand{\cmd}[1]{\texttt{#1}\xspace}
\newcommand{\AND}{\cmd{AND}}
\newcommand{\SAND}{\cmd{SAND}}
\newcommand{\OR}{\cmd{OR}}

% Table helpers
\newcommand{\xrule}[1]{\vspace{-6pt}\newline\rule[-1pt]{#1}{\lightrulewidth}}
\renewcommand{\arraystretch}{0.75}

\usepackage{upgreek}
\newcommand{\iface}{\ensuremath\dot\upiota}
\newcommand{\asset}{\ensuremath{A}}
\newcommand{\spgraph}[1]{\ensuremath{\llbracket #1 \rrbracket_{\mathcal{SP}}}}

% In order to tell LATEX to place figures within the text and not at the end of a chapter (which is the default), we adjust the 'float placement' parameters in the preamble to our document. Here are some useful values.

\renewcommand\topfraction{.9}
\renewcommand\textfraction{0.35}
\renewcommand\floatpagefraction{0.8}

\newcommand{\rev}[1]{#1}
